Towers and Bratteli-Vershik systems in Fibonacci-like unimodal maps

For a class of Fibonacci-like unimodal maps, the restriction to the $\omega$-limit set of the unique turning point defines a minimal Cantor system. We construct these Cantor sets geometrically using a nested sequence of finite covers with a tower structure. From this tower structure, we recover the associated Bratteli-Vershik model determined by the cutting times and obtain an explicit formula for the unique ergodic invariant probability measure supported on the $\omega$-limit set. We conclude with applications illustrating the scope of the construction.

==> The_post-critical_set.tex <==
\section{The set $\overline{\cO_T(c)}$}
\label{sec:post-critical}
\subsection{The combinatorics of the set $\overline{\cO_T(c)}$}
In this section we will give an explicit description of the set $\overline{\cO_{T(c)}}$  following \cite{LyMi93}.

Put  $S(-2) = 0$ and $S(-1) = 1$.
From (\ref{eq:cut_time}) we obtain that for every $k \geq 0$ the points $c_{S(k)}$ and $c_{S(k+2)}$ are on opposite sides of $c$. Since \[ c_{S(1)} = c_2 < c < c_1 =c_{S(0)}, \]
we conclude that for $k \equiv 0 \pmod 4,~c_{S(k)}$ is to the right of $c$ and if $k \equiv 2 \pmod4 $,~$c_{S(k)}$ is to the left of $c$. Since we also know that $c_{S(1)}$ is to
the left of $c$, we can conclude that for $k \equiv 1 \pmod 4$, $c_{S(k)}$ is to the left of $c$, and for $k \equiv 3 \pmod 4$, $c_{S(k)}$ is to the right of $c$. From this, we can
conclude that if $k$ is even the points $c_{S(k)}$ and $c_{S(k+1)}$ are in opposite sides of $c$, and therefore \[ [c_{S(k+1)}, c_{S(k)}]  \supseteq [c_{S(k+2)} , c_{S(k)}].  \] In the
case that $k$ is odd, $c_{S(k)}$ and $c_{S(k+1)}$ are on the same side with respect to $c$, and therefore \[ [c_{S(k+1)} , c_{S(k)}] \subseteq [c_{S(k+2)} , c_{S(k)}].  \]

For each $k \geq 0$ let $I_k$ be the smallest closed interval containing all of the points $c_{S(l)}$ for every $l \geq k$. For each $n \geq 0$ define $I^n_k \= T^n(I_k)$. By the
above discussion  
\begin{equation}
  \label{eq:I_K}
  I_k =
  \begin{cases}
    [c_{S(k)} , c_{S(k+1)}] \text{ if  $k$ is even, } \\
    [c_{S(k)}, c_{S(k+2)}]  \text{ if $k$ is odd. }
  \end{cases}
\end{equation}

\begin{lemm}
  \label{lemm:T_injective}
  For every $k \geq 1$, we have that $T^j$ is injective on $[c_1,c_{S(k)+1}]$. In particular $I_k^{j+1} = [c_{j+1},c_{S(k) + 1 + j}]$ for every $j \in \{1, \ldots, S(k-1)-1 \}.$ 
\end{lemm}
\begin{proof}
Since $|c - c_{S(k)}| > |c - c_{S(m)}|$  and $|T([c_{S(k)},c])| = \lambda|c - c_{S(k)}|$, for every $0 \leq k < m$ we get that $c_{S(k) +1} < c_{S(m) + 1} < c_1$, in particular
$I^1_k = [c_1, c_{S(k) +1}]$. In the case $k \geq 1$, by
(\ref{eq:cut_time}), with $k$ replaced by $k+1$, for every $j \in \{ 1, \ldots , S(k-1)-1 \}$ we have that $c_{S(k)+j}$ and $c_j$ are in the same side respect to $c$. Thus
$c \notin [c_{S(k) + j}, c_j] = T^{j-1}[c_{S(k) +1} , c_1]$, and then the map $T^j$ is injective on $[c_1, c_{S(k) +1}]$. In particular, for $1 < j \leq S(k-1)$

\begin{eqnarray}
  \label{eq:interval_image_general}
  I^{j}_k & = & T^{j-1}([c_1, c_{S(k)+1}])  \\
        & = & [c_j, c_{S(k) + j}] \nonumber 
\end{eqnarray}
\end{proof}
Note that for $k \geq 1$, by Lemma \ref{lemm:T_injective}, with $j = S(k-1) -1$
\begin{equation}
  \label{eq:interval_image}
  I_k^{S(k-1)} = [c_{S(k-1)}, c_{S(k) + S(k-1)}] = [c_{S(k-1)}, c_{S(k+1)}].
\end{equation}
Then, by (\ref{eq:cut_time}), $c \in I^{S(k-1)}_k$ and $c \notin I^n_k  $ for every $0 < n < S(k-1)$.
\begin{lemm} 
  \label{lemm:orbit_order}
  For all $k  \geq 0$ we have that \[ |c_i - c| > |c_{S(k-1)} - c|,\] for all $ 0 < i < S(k)$, with $i \neq S(k-1).$ 
\end{lemm}

\begin{proof}
  We will use induction on $k$. The cases $k = 0\text{ and } 1$ are vacuously true, the cases $k = 2 \text{ and } 3$ are true by the definition of Fibonacci map and
  (\ref{def:fibonacci_2}).
  Suppose now that it is true for $k$. We will prove that is
  true for $k+1$. \newline
  \textbf{Case 1:}
  Since \[ |c_{S(k-1)} - c| > |c_{S(k)} - c|,\] we have that  \[ |c_i - c| > |c_{S(k)} - c|,  \] for all $0 < i < S(k)$.\newline
  \textbf{Case 2:} 
  Since \[ c_{S(k-1) +1} < c_{S(k) +1} < c_1 \] and $T^i$ is injective on $[c_{S(k-1) +1},c_1]$ for $0<i<S(k-2)$ by Lemma \ref{lemm:T_injective}, we have that
  $c_{S(k) +i} \in (c_{S(k-1) + i}, c_i)$, for $0 < i < S(k-2)$. By the induction hypothesis, \[ |c_i -c|>|c_{S(k-1)}-c|>|c_{S(k)} -c| \]
  and \[ |c_{S(k-1) + i} - c|>|c_{S(k-1)} - c|>|c_{S(k)} - c|, \] for $0 < i < S(k-2).$ By \ref{eq:cut_time}
  $c_i$ and $c_{S(k-1) +i}$ lie on the same side of $c$ for $0 < i < S(k-2)$.  The above implies
  that \[ |c_{S(k) + i} - c| > |c_{S(k)} - c| \] for all $0 < i < S(k-2)$.\newline
  \textbf{Case 3:}
  Since $T^{S(k-2) -1}$ is injective on $[c_{S(k-1)+1}, c_1]$ we get that $c_{S(k)+S(k-2)} \in (c_{S(k)}, c_{S(k-2)})$. Also, by (\ref{eq:cut_time}),  $c_{S(k) +S(k-2)}$ and $c_{S(k-2)}$ lie on
  the same side of $c$, and opposite to $c_{S(k)}$. Then \[ |c_{S(k) + S(k-2)} - c|<|c_{S(k-2)} - c|.\]
  Hence \[ c_{S(k-2) + 1} < c_{S(k) + S(k-2) +1} < c_1. \] So by Lemma \ref{lemm:T_injective}, $c_{S(k) + S(k-2) +i} \in (c_{S(k-2)+i} , c_i)$ for
  $0 < i < S(k-3)$. By the induction hypothesis \[ |c_i - c|>|c_{S(k)} - c| \hspace{10pt} \text{ and } \hspace{10pt} |c_{S(k-2) + i} - c|>|c_{S(k)} - c|, \] for $0<i<S(k-3).$ Since, by
  (\ref{eq:cut_time}), $c_{S(k-2) +i}$ and $c_i$ lie on the same side of $c$ for $0<i<S(k-3)$ we get \[ |c_{S(k) + S(k-2) +i} -c| > |c_{S(k)} - c|, \] for all $0<i<S(k-3).$ \newline
  \textbf{Case 4:} It remains to prove that \[ |c_{S(k) + S(k-2)} - c|>|c_{S(k)} - c|.\]
  Suppose by contradiction that \[ |c_{S(k) + S(k-2)} - c|<|c_{S(k)} - c|.\] Then $c_{S(k) +1} < c_{S(k) + S(k-2) +1} < c_ 1$. Since $T^{S(k-3) -1}$ is injective on
  $[c_{S(k) +1}, c_1]$ we get that $c_{S(k+1)} \in (c_{S(k-3)},c_{S(k) + S(k-3)})$. Noting that by (\ref{eq:cut_time}) $c_{S(k-3)}$ and $c_{S(k) + S(k-3)}$ are in the same side with respect to
  $c$ we have either \[|c_{S(k+1)}-c|>|c_{S(k) + S(k-3)}-c|>|c_{S(k)}-c| \] or \[|c_{S(k+1)}-c|>|c_{S(k-3)}-c|>|c_{S(k)}-c|, \]
  a contradiction. So we must have \[ |c_{S(k) + S(k-2)}-c|>|c_{S(k)}-c|, \] and this conclude the proof.
 \end{proof}
 Let us denote \[ J_k \= I_{k+1}^{S(k-1)} = [c_{S(k-1)}, c_{S(k+1) + S(k-1)}],\] and put \[ D_k \= [c,c_{S(k)}] \] for every $k \geq 1$. For every $n \geq 0$ we use the notation
 \begin{equation}
   \label{eq:J_k_definition}
   J^n_k \= T^n(J_k) = I^{S(k-1) + n}_{k+1}.
\end{equation}
 Note that by definition $D_{k'} \subset [c_{S(k)},c_{S(k+2)}]$, for every $k' \geq k \geq 1.$ See figure \ref{fig:2}. 
 
 \begin{figure}[h!]
  \centering
    \begin{tikzpicture}[line cap=round,line join=round,>=triangle 45,x=3.3cm,y=4cm]
% \draw [color=cqcqcq,, xstep=0.2cm,ystep=0.2cm] (-1.7550529850375236,-1.6113667903735556) grid (2.098096250198763,0.5404792048718992);
\clip(-1.7606566481216794,-1.0290389905687337) rectangle (2.06076906654733,0.3050905534000426);
\draw [line width=2pt] (-1.6283250703999999,0)-- (1.87052,0);
\draw [line width=2pt] (-1.6283250703999999,-0.2)-- (0.2812059514774783,-0.2);
\draw [line width=1.5pt,dash pattern=on 1pt off 2pt] (0,-0.1)-- (1.87052,-0.1);
\draw [line width=1.5pt,dash pattern=on 1pt off 2pt] (-1.6283250703999999,-0.3)-- (0,-0.3);
\draw [line width=2pt] (-0.7809225348931643,-0.4)-- (0.2812059514774783,-0.4);
\draw [line width=1.5pt,dash pattern=on 1pt off 2pt] (-0.7809225348931643,-0.5)-- (0,-0.5);
\draw [line width=2pt] (-0.1,-0.6)-- (0.2812059514774783,-0.6);
\draw [line width=2pt] (-0.1,-0.8)-- (0.1582716909839456,-0.8);
\draw [line width=1.5pt,dash pattern=on 1pt off 2pt] (0,-0.7)-- (0.2812059514774783,-0.7);
\draw [line width=2pt] (0,0.08193371459071828)-- (0,-0.95);
\draw [line width=1.5pt,dash pattern=on 1pt off 2pt] (-0.1,-0.9)-- (0,-0.9);
\begin{scriptsize}
\draw [fill=black] (1.87052,0) circle (1pt);
\draw[color=black] (1.9165342443499325,0.06135724499302839) node {$c_{1}$};
\draw [fill=black] (-1.6283250703999999,0) circle (1pt);
\draw[color=black] (-1.6502154979238352,0.06135724499302839) node {$c_{2}$};
\draw [fill=black] (1.87052,-0.1) circle (1pt);
\draw[color=black] (1.9165342443499325,-0.04414827666653128) node {$c_{1}$};
\draw [fill=black] (-1.6283250703999999,-0.2) circle (1pt);
\draw[color=black] (-1.6502154979238352,-0.13701605769366196) node {$c_{2}$};
\draw [fill=black] (0,-0.1) circle (1pt);
\draw[color=black] (0.0471180359804952,-0.03614827666653128) node {};
\draw [fill=black] (0.2812059514774783,-0.2) circle (1pt);
\draw[color=black] (0.32954782285645334,-0.16701605769366196) node {$c_{5}$};
\draw [fill=black] (-1.6283250703999999,-0.3) circle (1pt);
\draw[color=black] (-1.6502154979238352,-0.25788383872079263) node {$c_{2}$};
\draw [fill=black] (-0.7809225348931643,-0.4) circle (1pt);
\draw[color=black] (-0.8029261372959607,-0.35875161974792334) node {$c_{3}$};
\draw [fill=black] (0.2812059514774783,-0.4) circle (1pt);
\draw[color=black] (0.32954782285645334,-0.33875161974792334) node {$c_{5}$};
\draw [fill=black] (0,-0.3) circle (1pt);
\draw[color=black] (0.0471180359804952,-0.23788383872079263) node {};
\draw[color=black] (0.1345367795373394,0.082612461093534123) node {$I_0$};
\draw[color=black] (-0.6623186905769711,-0.13434802314779552) node {$I_1$};
\draw[color=black] (0.9482035464895046,-0.16348024212066482) node {$D_0$};
\draw[color=black] (-1.0335335840149502,-0.35185354480735517) node {$D_1$};
\draw[color=black] (0.1386740102630339,-0.35272132583448584) node {$I_2$};
\draw [fill=black] (-0.7809225348931643,-0.5) circle (1pt);
\draw[color=black] (-0.8029261372959607,-0.45625714140748295) node {$c_{3}$};
\draw [fill=black] (0,-0.5) circle (1pt);
\draw[color=black] (0.05552368439942253,-0.43625714140748295) node {};
\draw [fill=black] (-0.1,-0.6) circle (1pt);
\draw[color=black] (-0.115344096627705395,-0.5671249224346136) node {$c_{13}$};
\draw [fill=black] (0.2812059514774783,-0.6) circle (1pt);
\draw[color=black] (0.32954782285645334,-0.5371249224346136) node {$c_{5}$};
\draw[color=black] (-0.379888903701013,-0.5435891068616165) node {$D_2$};
\draw[color=black] (0.10091418586163009,-0.5544568878887472) node {$I_3$};
\draw [fill=black] (-0.1,-0.8) circle (1pt);
\draw[color=black] (-0.115344096627705395,-0.7688604844888751) node {$c_{13}$};
\draw [fill=black] (0.1582716909839456,-0.8) circle (1pt);
\draw[color=black] (0.20514422625632892,-0.7688604844888751) node {$c_{8}$};
\draw [fill=black] (0,-0.7) circle (1pt);
\draw[color=black] (0.05552368439942253,-0.6379927034617443) node {};
\draw [fill=black] (0.2812059514774783,-0.7) circle (1pt);
\draw[color=black] (0.32954782285645334,-0.6679927034617443) node {$c_{5}$};
\draw[color=black] (0.06039351724535334,-0.7528301905754376) node {$I_4$};
\draw[color=black] (0.15134807637519404,-0.6619624095483069) node {$D_3$};
\draw[color=black] (-0.03357618884120714,-0.3824609915263466) node {};
\draw [fill=black] (0,0.08193371459071828) circle (1pt);
\draw[color=black] (-0.026944479775069613,0.1353269510795909) node {$c$};
\draw [fill=black] (-0.1,-0.9) circle (1pt);
\draw[color=black] (-0.115344096627705395,-0.8663660061484347) node {$c_{13}$};
\draw[color=black] (-0.08693844820877806,-0.9536979716025683) node {$D_5$};
\end{scriptsize}
\end{tikzpicture}

 \caption{First five $I_k$ (solid line), and $D_k$ (dashed line) intervals.}
  \label{fig:2}
\end{figure}
 
 \begin{lemm}
  \label{lemm:J_k}
  For all $0< k <k'$ we have $J_{k'} \subset D_{k'-1} \subset I_{k}$ and $J_{k} \cap J_{k'} = \emptyset$.
\end{lemm}
\begin{proof}
  First we will prove that $J_{k+1}$ is contained in $D_k$ and $c \notin J_{k+1}$ for every $k \geq 0$. Fix $k \geq 0$.
  By (\ref{eq:cut_time}) with $k$ replaced by $k+3$ we have $c_{S(k)}$ and $c_{S(k+2) + S(k)}$ are in the same side of $c$. Since \[ |c_{S(k+2)} - c| < |c_{S(k+1)} -c|,\] we have
  \[c_{S(k+1) +1}<c_{S(k+2) +1}<c_1.\] By Lemma \ref{lemm:T_injective}, $T^{S(k) -1}$ is injective on $I_{k+1}^1$. Then, $c_{S(k+2) + S(k)} \in (c_{S(k+2)} , c_{S(k)})$. By (\ref{eq:cut_time})
  with $k$ replaced by $k+3$, we thus conclude $c_{S(k+2) + S(k)} \in (c_{S(k)} , c)$. Then
  \[J_{k+1} = [c_{S(k)}, c_{S(k) + S(k+2)}] \subset [c, c_{S(k)}] = D_k\subset [c_{S(k)},c_{S(k+2)}] \subseteq I_k \] and $c \notin J_{k+1}$. Since, by definition, for every $k' > k$ we have
  $D_{k'-1} \subset I_{k'-1} \subset I_k$, we get \[ J_{k'} \subset D_{k'-1} \subset I_k.  \]
  Now we will prove that $J_{k+1}$ and $I_{k+1}$ are disjoint.
  If $k$ is even then $I_{k+1} = [c_{S(k+1)} , c_{S(k+3)}]$. Since $c_{S(k)}$ and $c_{S(k+1)}$ lie on opposite sides respect to $c$, we have that $c_{S(k)}$, $c_{S(k) + S(k+2)}$, and
  $c_{S(k+3)}$ lie on the same side of $c$. By (\ref{lemm:orbit_order}), with $k$ replaced by $k+4$, we get \[ |c_{S(k)} - c|>|c_{S(k) + S_{k+2}} - c|>|c_{S(k+3)} - c|. \] So
  $J_{k+1} \cap I_{k+1} = \emptyset.$ Now, if $k$ is odd $I_{k+1} = [c_{S(k+1)}, c_{S(k+2)}]$ and $c_{S(k)}$, $c_{s(k+1)}$ and $c_{S(k) + S(k+2)}$ lie on the same side of $c$. Suppose that
  $|c_{S(k+1)} - c| > |c_{S(k) + S(k+2)} - c|$, then \[[c_{S(k+1)},c_{S(k) + S(k+2)}] \subset [c_{S(k)},c_{S(k) + S(k+2)}].\] Since $T^{S(k-1)}$ is injective on $[c_{S(k)},c_{S(k) + S(k+2)}]$, then
  $T^{S(k-1)}$ is injective on \newline $[c_{S(k+1)},c_{S(k) + S(k+2)}]$. So we get \[T^{S(k-1)}([c_{S(k+1)},c_{S(k) + S(k+2)}]) = [c_{S(k+1)+S(k-1)},c_{S(k+3)}].\] Since
  $S(k+1) + S(k-1) < S(k+4),$ by
  Lemma \ref{lemm:orbit_order}, with $k$ replaced by $k+4$, we get \[|c_{S(k+1) + S(k-1)} - c|>|c_{S(k+3)} - c|.\] On the other hand, $T^{S(k-1)}(J_{k+1}) = [c_{S(k+1)}, c_{S(k+3)}]$, then
  \[T^{S(k-1)}(c_{S(k+1)}) = c_{S(k+1) + S(k-1)} \in (c_{S(k+1)} , c_{S(k+3)})\] and by (\ref{eq:cut_time}), with $k$ replaced by $k+1$, we have that $c_{S(k+1) + S(k-1)}$ and $c_{S(k-1)}$ are in
  the same side of $c$. Since $k-1 \equiv k+3  \pmod4$, we have that $c_{S(k-1)}$ and $c_{S(k+3)}$ are on the same side of $c$, so
  $c_{S(k+1) + S(k-1)} \in (c,c_{S(k+3)})$. Thus \[ |c_{S(k+1) + S(k-1)} - c|<|c_{S(k+3)} - c|, \] a contradiction. So we must have $c_{S(k) + S(k+2)} \in (c_{S(k)}, c_{S(k+1)})$ and
  \begin{equation}
    \label{eq:empty_intersection}
    J_{k+1}~\cap~I_{k+1}~=~\emptyset. 
  \end{equation}
  This conclude the proof of the lemma.
\end{proof}

Taking $k' = k+1$ in Lemma \ref{lemm:J_k} we get $J_{k+1} \subset I_k$, and then 
\begin{equation}
  \label{eq:J_k_I_k_1}
  J_{k+1} \cup I_{k+1} \subset I_k \subseteq I_k^{S(k-1)},
\end{equation}
for every $k \geq 1$
\begin{defi}
  For $k \geq 0$ let $M_k$ be the $S(k)-$fold union \[ M_k = \bigcup_{0 \leq n < S(k-1) } I^n_k \cup \bigcup_{0 \leq n < S(k-2)} J^n_k.  \]
\end{defi}

\noindent Some examples of $M_k$,
\begin{eqnarray}
  M_0 & = & I_0 \nonumber \\
      & = & [c_1, c_2], \nonumber \\
  M_1 & = & I_1 \cup J_1 \nonumber \\
      & = & [c_2, c_5] \cup [c_4,c_1], \nonumber \\
  M_2 & = & I_2 \cup I^1_2 \cup J_2 \nonumber \\
      & = & [c_3, c_5] \cup [c_4, c_1] \cup [c_2,c_7] \nonumber \\
  M_3 & = & I_3 \cup I^1_3 \cup I^2_3 \cup J_3 \cup J^1_3 \nonumber \\
      & = & [c_{13}, c_5] \cup [c_6, c_1] \cup [c_2, c_7] \cup [c_3, c_{11}] \cup [c_4, c_{12}] \nonumber \\
  M_4 & = & I_4 \cup I^1_4 \cup I^2_4 \cup I^3_4 \cup I^4_4 \cup J_4 \cup J^1_4 \cup J^2_4 \nonumber \\
      &= & [c_{13}, c_8] \cup [c_9, c_1] \cup [c_2, c_{10}] \cup [c_3, c_{11}] \cup [c_4, c_{12}] \cup [c_{14}, c_5] \cup [c_6, c_{19}] \cup [c_{20}, c_7], \nonumber 
\end{eqnarray}
\noindent and so on. 

\begin{figure}[h!]
  \centering
    \begin{tikzpicture}[line cap=round,line join=round,>=triangle 45,x=3.3cm,y=4cm]
    \clip(-1.7606566481216794,-1.0290389905687337) rectangle (2.06076906654733,0.3050905534000426);
\draw [line width=2pt] (-1.6283250703999999,0)-- (1.87052,0);
\draw [line width=2pt] (-1.6283250703999999,-0.2)-- (0.34,-0.2);
\draw [line width=2pt] (1.15,-0.2)-- (1.87052,-0.2);
\draw [line width=2pt] (-1.6283250703999999,-0.4)-- (-1.26,-0.4);
\draw [line width=2pt] (-0.7809225348931643,-0.4)-- (0.34,-0.4);
\draw [line width=2pt] (1.15,-0.4)-- (1.87052,-0.4);
\draw [line width=2pt] (-1.6283250703999999,-0.6)-- (-1.26,-0.6);
\draw [line width=2pt] (-0.7809225348931643,-0.6)-- (-0.58,-0.6);
\draw [line width=2pt] (-0.1,-0.6)-- (0.34,-0.6);
\draw [line width=2pt] (1.15,-0.6)-- (1.44,-0.6);
\draw [line width=2pt] (1.6,-0.6)-- (1.87052,-0.6);
\draw [line width=2pt] (-1.6283250703999999,-0.8)-- (-1.5462762185432146,-0.8006740305557355);
\draw [line width=2pt] (-1.4,-0.8)-- (-1.26,-0.8);
\draw [line width=2pt] (-0.7809225348931643,-0.8)-- (-0.58,-0.8);
\draw [line width=2pt] (-0.1,-0.8)-- (0.1182716909839456,-0.8);
\draw [line width=2pt] (0.19,-0.8)-- (0.34,-0.8);
\draw [line width=2pt] (1.15,-0.8)-- (1.44,-0.8);
\draw [line width=2pt] (1.6,-0.8)-- (1.68,-0.8);
\draw [line width=2pt] (1.8,-0.8)-- (1.87052,-0.8);
\draw [line width=2pt] (0,0.08193371459071828)-- (0,-0.85);
\begin{scriptsize}
\draw [fill=black] (1.87052,0) circle (1pt);
\draw[color=black] (1.917382237811931,0.06325904625025687) node {$c_{1}$};
\draw [fill=black] (-1.6283250703999999,0) circle (1pt);
\draw[color=black] (-1.6505894678493178,0.06325904625025687) node {$c_{2}$};
\draw [fill=black] (1.87052,-0.2) circle (1pt);
\draw[color=black] (1.917382237811931,-0.1368155984968159) node {$c_{1}$};
\draw [fill=black] (-1.6283250703999999,-0.2) circle (1pt);
\draw[color=black] (-1.6505894678493178,-0.1368155984968159) node {$c_{2}$};
\draw [fill=black] (1.15,-0.2) circle (1pt);
\draw[color=black] (1.127113516722484,-0.1368155984968159) node {$c_{4}$};
\draw [fill=black] (0.34,-0.2) circle (1pt);
\draw[color=black] (0.38681120549685644,-0.1368155984968159) node {$c_{5}$};
\draw [fill=black] (1.87052,-0.4) circle (1pt);
\draw[color=black] (1.917382237811931,-0.33689024324388867) node {$c_{1}$};
\draw [fill=black] (-1.6283250703999999,-0.4) circle (1pt);
\draw[color=black] (-1.6505894678493178,-0.33689024324388867) node {$c_{2}$};
\draw [fill=black] (-0.7809225348931643,-0.4) circle (1pt);
\draw[color=black] (-0.8036068050867275,-0.33689024324388867) node {$c_{3}$};
\draw [fill=black] (1.15,-0.4) circle (1pt);
\draw[color=black] (1.127113516722484,-0.33689024324388867) node {$c_{4}$};
\draw [fill=black] (0.34,-0.4) circle (1pt);
\draw[color=black] (0.38681120549685644,-0.33689024324388867) node {$c_{5}$};
\draw [fill=black] (-1.26,-0.4) circle (1pt);
\draw[color=black] (-1.2137859524796921,-0.33689024324388867) node {$c_{7}$};
\draw[color=black] (0.13338332215056958,0.0513436234236121024) node {$I_0$};
\draw[color=black] (-0.6618998026278329,-0.14059826405963703) node {$I_1$};
\draw[color=black] (1.5773910588998377,-0.14059826405963703) node {$J_1$};
\draw[color=black] (-1.4732370712972787,-0.3455645576149869) node {$J_2$};
\draw[color=black] (-0.24000442291972096,-0.3455645576149869) node {$I_2$};
\draw[color=black] (1.5773910588998377,-0.3405645576149869) node {$I_2^1$};
% \draw[color=black] (-0.6335694827131932,-0.2135108789831938) node {$g$};
% \draw[color=black] (1.520567525730245,-0.2135108789831938) node {$h$};
% \draw[color=black] (-1.4338680617014676,-0.4135855237302666) node {$i$};
% \draw[color=black] (-0.2100781513318981,-0.4135855237302666) node {$j$};
% \draw[color=black] (1.520567525730245,-0.4135855237302666) node {$k$};
\draw [fill=black] (-1.6283250703999999,-0.6) circle (1pt);
\draw[color=black] (-1.6505894678493178,-0.5369648879909615) node {$c_{2}$};
\draw [fill=black] (-1.26,-0.6) circle (1pt);
\draw[color=black] (-1.2137859524796921,-0.5369648879909615) node {$c_{7}$};
\draw [fill=black] (-0.7809225348931643,-0.6) circle (1pt);
\draw[color=black] (-0.8036068050867275,-0.5369648879909615) node {$c_{3}$};
\draw [fill=black] (-0.58,-0.6) circle (1pt);
\draw[color=black] (-0.525195716808531,-0.5369648879909615) node {$c_{11}$};
\draw [fill=black] (-0.1,-0.6) circle (1pt);
\draw[color=black] (-0.125016569415566546,-0.5369648879909615) node {$c_{13}$};
\draw [fill=black] (0.34,-0.6) circle (1pt);
\draw[color=black] (0.38681120549685644,-0.5369648879909615) node {$c_{5}$};
\draw [fill=black] (1.15,-0.6) circle (1pt);
\draw[color=black] (1.127113516722484,-0.5369648879909615) node {$c_{4}$};
\draw [fill=black] (1.44,-0.6) circle (1pt);
\draw[color=black] (1.4555581951368613,-0.5369648879909615) node {$c_{12}$};
\draw [fill=black] (1.6,-0.6) circle (1pt);
\draw[color=black] (1.5872814674033882,-0.5369648879909615) node {$c_{6}$};
\draw [fill=black] (1.87052,-0.6) circle (1pt);
\draw[color=black] (1.917382237811931,-0.5369648879909615) node {$c_{1}$};
\draw[color=black] (-1.4732370712972787,-0.5337762002450147) node {$I_3^2$};
\draw[color=black] (-0.6805800387479996,-0.5337762002450147) node {$J_3$};
\draw[color=black] (0.10075722992144626,-0.5337762002450147) node {$I_3$};
\draw[color=black] (1.293198019971104,-0.5337762002450147) node {$J_3^1$};
\draw[color=black] (1.7286027015298602,-0.5337762002450147) node {$I_3^1$};
% \draw[color=black] (-1.4338680617014676,-0.6136601684773394) node {$l$};
% \draw[color=black] (-0.6702498342501558,-0.6136601684773394) node {$m$};
% \draw[color=black] (0.13004874473811845,-0.6136601684773394) node {$n$};
% \draw[color=black] (1.3071545713333719,-0.6136601684773394) node {$p$};
% \draw[color=black] (1.7473187897769227,-0.6136601684773394) node {$q$};
\draw [fill=black] (-1.6283250703999999,-0.8) circle (1pt);
\draw[color=black] (-1.6505894678493178,-0.7370395327380342) node {$c_{2}$};
\draw [fill=black] (-1.5462762185432146,-0.8006740305557355) circle (1pt);
\draw[color=black] (-1.5222231664193626,-0.7403741101504855) node {$c_{10}$};
\draw [fill=black] (-1.26,-0.8) circle (1pt);
\draw[color=black] (-1.2054495089485642,-0.7370395327380342) node {$c_{7}$};
\draw [fill=black] (-1.4,-0.8) circle (1pt);
\draw[color=black] (-1.3954980280341588,-0.7370395327380342) node {$c_{20}$};
\draw [fill=black] (-0.7809225348931643,-0.8) circle (1pt);
\draw[color=black] (-0.8136105373240809,-0.7370395327380342) node {$c_{3}$};
\draw [fill=black] (-0.58,-0.8) circle (1pt);
\draw[color=black] (-0.525195716808531,-0.7370395327380342) node {$c_{11}$};
\draw [fill=black] (-0.1,-0.8) circle (1pt);
\draw[color=black] (-0.115016569415566546,-0.7370395327380342) node {$c_{13}$};
\draw [fill=black] (0.1182716909839456,-0.8) circle (1pt);
\draw[color=black] (0.09337958991321615,-0.7370395327380342) node {$c_{8}$};
\draw [fill=black] (0.19,-0.8) circle (1pt);
\draw[color=black] (0.19509166546768288,-0.7370395327380342) node {$c_{18}$};
\draw [fill=black] (0.34,-0.8) circle (1pt);
\draw[color=black] (0.38681120549685644,-0.7370395327380342) node {$c_{5}$};
\draw [fill=black] (1.15,-0.8) circle (1pt);
\draw[color=black] (1.127113516722484,-0.7370395327380342) node {$c_{4}$};
\draw [fill=black] (1.44,-0.8) circle (1pt);
\draw[color=black] (1.455581951368613,-0.7370395327380342) node {$c_{12}$};
\draw [fill=black] (1.6,-0.8) circle (1pt);
\draw[color=black] (1.5772814674033882,-0.7370395327380342) node {$c_{6}$};
\draw [fill=black] (1.68,-0.8) circle (1pt);
\draw[color=black] (1.6956477688333436,-0.7370395327380342) node {$c_{19}$};
\draw [fill=black] (1.8,-0.8) circle (1pt);
\draw[color=black] (1.807356112150457,-0.7370395327380342) node {$c_{9}$};
\draw [fill=black] (1.87052,-0.8) circle (1pt);
\draw[color=black] (1.917382237811931,-0.7370395327380342) node {$c_{1}$};
\draw[color=black] (-1.5772548904368666,-0.8737348132244122) node {$I_4^2$};
\draw[color=black] (-1.3171578522656775,-0.8737348132244122) node {$J_4^2$};
\draw[color=black] (-0.6702498342501558,-0.8737348132244122) node {$I_4^3$};
\draw[color=black] (-0.05,-0.8737348132244122) node {$I_4$};
\draw[color=black] (0.27677015088596874,-0.8737348132244122) node {$J_4$};
\draw[color=black] (1.3071545713333719,-0.8737348132244122) node {$I_4^4$};
\draw[color=black] (1.6506160448158396,-0.8737348132244122) node {$J_4^1$};
\draw[color=black] (1.847356112150457,-0.8737348132244122) node {$I_4^1$};
\draw[color=black] (-0.03334554847198755,-0.3335556658314375) node {};
\draw [fill=black] (0,0.08193371459071828) circle (1pt);
\draw[color=black] (0.026676844952133016,0.13328517191173234) node {$c$};
\end{scriptsize}
\end{tikzpicture}
   \caption{First five levels of $M_k$.}
  \label{fig:3}
\end{figure}

From the definition, for every $k \geq 0$ the $S(k)$ closed intervals \[ I_k, I^1_k, \ldots , I^{S(k-1) -1}_k, J_k, J^1_k, \ldots , J^{S(k-2)-1}_k,\] are pairwise disjoint, each $M_k$
contains the set $\overline{\cO_T(c)}$ and they
form a nested sequence of closed sets $M_1 \supset M_2 \supset M_3 \supset \ldots$ with intersection equal to the Cantor set $\overline{\cO_T(c)}$, for a proof of these
statements see \cite[Lemma 3.5]{LyMi93}.
Now by (\ref{eq:J_k_I_k_1}) we have that for every $1 \leq m < S(k-1)$, \[ I_{k+1}^m \cup J_{k+1}^m \subset I_k^m. \] Also by (\ref{eq:J_k_definition}) for every $0 \leq n < S(k-2)$,
\[ I_{k+1}^{S(k-1) + n} = J_k^n. \] Since the sets in $M_k$ are disjoint we get that
\begin{equation}
  \label{eq:J_k_I_k}
  \cup_{A \in M_{k+1}} (A \cap I_k) = I_{k+1} \cup J_{k+1.} 
\end{equation}

\subsection{Diameter estimates}
In this section we will give an estimate on how the distances $|c_{S(k)} - c|$ decrease as $k \to \infty.$
 
\begin{lemm}
  \label{lemm:diam_estimate}
  The following limit \[ \lim_{k \to \infty} \lambda^{S(k+1)}|D_k|\] exists and is strictly positive. 
\end{lemm}

\begin{proof}
  Since \[T(D_k) = T([c,c_{S(k)}]) = I_k^1,\] by (\ref{eq:interval_image}) we have that \[T^{S(k-1)}(D_k) = [c_{S(k-1)}, c_{S(k+1)}] .\]
  By (\ref{eq:cut_time}), $c_{S(k-1)}$ and $c_{S(k+1)}$ are in opposite sides of $c$. Then $D_{k-1} \cap D_{k+1} = \{c\}$, so \[T^{S(k-1)}(D_k) = D_{k-1} \cup D_{k+1} .\] Since, by
  Lemma~\ref{lemm:T_injective}, $T^{S(k-1)}$ is injective on $I_k$ and $D_k \subset I_k$ we get that \[ |T^{S(k-1)}(D_k)| = \lambda^{S(k-1)} |D_k| = |D_{k-1}| +|D_{k+1}|.\]
  For $k \geq 0$ put  $\nu_k\= |D_k| / |D_{k+1}|$. By the above we get \[ \lambda^{S(k-1)} = \nu_{k-1} + \frac{1}{\nu_k}. \] By (\ref{def:fibonacci}),
  $\nu_k > 1$, so $0 < \nu_k^{-1} <1$. Since
  $\lambda >1$, we have $\lambda^{S(k-1)} \longrightarrow \infty$ as $k \longrightarrow \infty$. Then $\nu_k \longrightarrow \infty$ as $k \longrightarrow \infty$. So
  $\lambda^{S(k-1)} - \nu_{k-1} \longrightarrow 0$ as $k \longrightarrow \infty.$ Then, if we define $C_k \=\nu_k\lambda^{-S(k)}$, we have $0 < C_k < 1$ and $C_k \nearrow 1$
  exponentially fast as $n \longrightarrow\infty.$ By definition of $\nu_k$, we have that
  \[ \frac{|D_0|}{|D_{k+1}|} = \prod_{i=0}^k \nu_i 
                            = \prod_{i=0}^k \lambda^{S(i)}C_i 
                            =\lambda^{S(k+2) - S(1)}\prod_{i=0}^k C_i. \]
  Then 
  \begin{equation}
    \label{eq:diameter_estimate}
    |D_{k+1}|\lambda^{S(k+2) - S(1)} = |D_0| \left[ \prod_{i = 0}^k C_i \right]^{-1}. 
  \end{equation}
  Since $ \prod_{i = 0}^k C_i $ converge to a strictly positive number as $k \longrightarrow \infty$, the proof is complete.
\end{proof}
%%% Local Variables:
%%% mode: latex
%%% TeX-master: "Unbounded_Lyapunov_exponent"
%%% End:

